Automatic Text Evaluation through the Lens of Wasserstein Barycenters

A new metric \texttt{BaryScore} to evaluate text generation based on deep contextualized embeddings e.g., BERT, Roberta, ELMo) is introduced. This metric is motivated by a new framework relying on optimal transport tools, i.e., Wasserstein distance and barycenter. By modelling the layer output of deep contextualized embeddings as a probability distribution rather than by a vector embedding; this framework provides a natural way to aggregate the different outputs through the Wasserstein space topology. In addition, it provides theoretical grounds to our metric and offers an alternative to available solutions e.g., MoverScore and BertScore). Numerical evaluation is performed on four different tasks: machine translation, summarization, data2text generation and image captioning. Our results show that \texttt{BaryScore} outperforms other BERT based metrics and exhibits more consistent behaviour in particular for text summarization.

==> image_captionning.tex <==
 \begin{table}
 \centering
 \begin{tabular}{lrr} \hline
  & M1 & M2 \\
      \cmidrule(lr){2-2} \cmidrule(lr){3-3}
     \texttt{BaryS}\textsuperscript{+} & 85.6 & 83.9 \\
      \texttt{BaryS}  & 85.2 & 82.6 \\
   \texttt{MoveS}\textsuperscript{+} & 83.1 & 82.6 \\
    \texttt{MoveS}  & 78.1 & 82.1 \\
  \texttt{BertS} - P & 83.0 & 82.1 \\
   \texttt{BertS} - R & 80.1 & 75.2 \\
    \texttt{BertS} - F & 79.1 & 81.1 \\\hline
         \texttt{BLEU}  & 58.3 & 60.8 \\
        \texttt{METEOR} & 60.3 & 59.9 \\ 
        \texttt{SPICE\textsuperscript{*}} & 75.9 & 75.0 \\\hline
        \texttt{CIDER\textsuperscript{*}} & 43.8 & 44.0 \\\hline
        
        \texttt{LEIC\textsuperscript{*}} & \textbf{93.9} & \textbf{94.9}\\\hline
%'bert score precision' & 0.8298596195547022 &   0.8286964643168034,\\ 
% 'bert score recall' & 0.8005453322389522  & 0.7521129632265942,\\ 
% 'bert score f1' & 0.7910606251594561 &  0.8109534421094943,\\ 
% 'bleu' & 0.5830029543470656 &   0.6082501168066831,\\ 
%mover score & 0.7818182816852614 &  0.8264373529678626,\\ 
%mover score + MNLI  & 0.8310993304912341 & 0.82617997796574018,\\ 
%bary score  & 0.8521344525522455 & 0.82617997796574018, \\ 
%bary score + MNLU & 0.8556425688988764 & 0.8387050388519908\\ 
\end{tabular}\caption{System level Pearson correlation with human judgement on the MSCOCO dataset.\footnote{Results with * are reported from \cite{zhao2019moverscore}}}\label{tab:captionning}
\end{table} % bert score uncased 



==> summarizatino_backup.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|ccc}
abs summ & $r$ & $\tau$	 & $\rho$ \\
R	recall &	0.735905 &	0.730703 &	0.745397 \\
bertscore f1 &	0.734724 &	0.749380 &	0.706321 \\
	R2	&	0.730127 &	0.735164 &	0.730066 \\
mover  &	0.724409 &	0.719189 &	0.730338 \\
mover  +MNLI &	0.733201 &	0.712379 &	0.730018 \\
recall bert  &	0.717968 &	0.719381 &	0.720869 \\
js-2 & 0.689995 &	0.68699 &	0.698072 \\
bary	  &	0.756868 &	0.759783 &	0.766869 \\
bary mnli  &	0.724968 &	0.734581 &	0.763269 \\\hline
abs sys &$r$ & $\tau$	 & $\rho$ \\
R2 &	0.985297 &	0.890110 &	0.960440 \\
js-2 &	0.925879 &	0.824176 &	0.929670 \\
bert score &		0.923161 &	0.824176 &	0.934066 \\
R1 & 	0.903665 &	0.802198 &	0.925275 \\
bary & 0.949420	&  0.834176& 	0.963253 \\
bary MNLI & 0.959122& 	0.834116&	0.962345 \\
mover score & 0.828517 &	0.758242 &	0.925275 \\
\textbf{mover score + MNLI} & 0.828517 &	0.758242 &	0.925275 \\
    \end{tabular}
    \caption{Abstractive}
    \label{tab:my_label}
\end{table}


\begin{table}[]
    \centering
    \begin{tabular}{c|ccc}
    ext sum & $r$ & $\tau$	 & $\rho$ \\
    bary score &	0.811685&	0.811685&	0.707704 \\
         \textbf{ bary score + MNLI} &	0.811685&	0.811685&	0.707704 \\
recall berts&	0.709320&	0.729620&	0.738920 \\
f1 berts &	0.294066	&0.189659&	0.550361\\
    mover score	&	0.761291 &	0.761291 &	0.474428 \\
        \textbf{mover score	+ MNLI} &	0.761291 &	0.761291 &	0.474428 \\
    js-2 & 0.055426	& 0.127273& 	0.190909\\ 
    R2&	0.722738&	0.740838&	0.691762\\
    R1&	0.551197&	0.532831&	0.690551\\ \hline
ext sys &$r$ & $\tau$	 & $\rho$ \\
R1 &	0.732751 &	0.527273 &	0.690909\\
R2 &	0.699662 &	0.418182 &	0.545455 \\
BERT score recall&	0.690213 &	0.490909 &	0.627273\\
BERT score f1 & 0.069095&	0.018182& 	0.027273 \\
BaryScore + MNLI &	0.640347 &	0.381818 &	0.481818\\
BaryScore   &	0.632235 &	0.418182 &	0.454545\\
moverscore & 	0.161596& 	0.090909& 	0.090909\\
moverscore + MNLI	& 0.211333& 	0.151231& 	0.290458\\
js-2 & 0.055426& 	0.127273	& 0.190909\\
   \end{tabular}
    \caption{Extractive} % roberta base
    \label{tab:my_label}
\end{table}



